Comprehensive and Efficient Workload Compression

This work studies the problem of constructing a representative workload from a given input analytical query workload where the former serves as an approximation with guarantees of the latter. We discuss our work in the context of workload analysis and monitoring. As an example, evolving system usage patterns in a database system can cause load imbalance and performance regressions which can be controlled by monitoring system usage patterns, i.e.,~a representative workload, over time. To construct such a workload in a principled manner, we formalize the notions of workload {\em representativity} and {\em coverage}. These metrics capture the intuition that the distribution of features in a compressed workload should match a target distribution, increasing representativity, and include common queries as well as outliers, increasing coverage. We show that solving this problem optimally is NP-hard and present a novel greedy algorithm that provides approximation guarantees. We compare our techniques to established algorithms in this problem space such as sampling and clustering, and demonstrate advantages and key trade-offs of our techniques.

==> experiments.tex <==
\section{Evaluation} \label{sec:eval}

In this section, we empirically evaluate the techniques discussed throughout this paper. We have implemented our summarization framework on top of a production DBMS \footnote{name omitted due to double blind restrictions} which supports fine grained logging of queries and easy AST parsing. The goal of this section is to evaluate the following:

\begin{packed_item}
    \item The time complexity of all algorithms for varying workloads and summary size constraints.
    \item A comparison of the coverage and representativity metrics of our solution with k-medoids, hierarchical clustering and random sampling both on real production workloads and using TPC-H workloads.
    \item The scalability of our solution on large scale workloads.
    \item The (smooth) trade-off between representativity and coverage metrics.
\end{packed_item}

\begin{table}[t]
	\begin{tabular}{ c|c|c|c} 
		\toprule[0.1em]
		feature & min value & max value & average 
		\\ \midrule[0.1em]
		exec time (sec) & $0$ & $21599$ & $0.0014$ \\
		cpu time (sec) & $0$ & $632$ & $0.114$ \\
		input size & $0$ & $115$ GB & $1.94$ KB \\
		output rows & $0$ & $298724$ & $1.0179$ \\
		planning time (sec) & $0$ & $234$ & $0.001425$\\
		\bottomrule
	\end{tabular}
	\caption{Workload statistics for \texttt{Adhoc}}
	\label{table:Adhoc}
\end{table}

\smallskip
\noindent \introparagraph{Benchmark Datasets} We perform our experiments over $2$ different datasets:

\begin{packed_enum}
    \item \texttt{AdHoc queries}: A dataset of ad-hoc visualization queries issued by production customers over System X. 
    This workload contains references $2729$ relations in total. 
    The largest join query contains $19$ joins and the workload has $106$ unique function calls. Other key information is shown in Table~\ref{table:Adhoc}.
    \item \texttt{TPC-H}~\cite{tpch} : A benchmark for performance metrics over systems operating at scale.
\end{packed_enum}

\begin{figure*}[t]
    \hspace{-1cm}
    \begin{subfigure}{0.45\linewidth}
    \includegraphics[scale=0.88]{figures/algorithms.pdf}
    \caption{runtime of algorithms} \label{fig:timetaken}
    \end{subfigure}
    \hspace{0.5cm}
    \begin{subfigure}{0.43\linewidth}
    \includegraphics[scale=1]{figures/metrics.pdf} 
    \caption{Coverage and Representativity} \label{fig:repcov}
    \end{subfigure}
    \caption{Experiments to show summary metrics and measure time complexity}
\end{figure*}

\smallskip
\noindent \introparagraph{Algorithms} For our experiments, we vary the following parameters: $(1)$ the algorithm for summarization (k-medoids, hierarchical clustering algorithm, random sampling and our algorithm), $(2)$ the features to be used, $(3)$ only for our algorithm, the desired output feature distribution (this could either be the input or the zipfian distribution). 
For the clustering algorithms, we implement two different distance functions: $(i)$ for categorical features, we calculate the Jaccard distance between the token list of each feature; and $(ii)$ for numeric features, we use the Euclidean distance between the normalized scores as the distance function. 
For both these variants, we also allow the weights to differ which helps us remove some features altogether by setting their weight to zero.

\begin{figure}[t]
    \includegraphics[width=\columnwidth]{figures/arch.pdf}
    \caption{Summarization framework architecture}
    \label{fig:arch}
\end{figure}

\smallskip
\noindent \introparagraph{Experimental Setup} The summarization framework is built as a layer that sits on top of the DBMS. 
It consists of two distinct modules: the analyzer module that is used to transform and materialize the feature vectors of all queries that have been executed on the DBMS and the summarizer module that uses the materialized feature vectors and the input from the user to generate the workload summary. 
Figure~\ref{fig:arch} shows the high level architecture of the modules. 
For both datasets, we assume that the workload has already been executed on the database and the logs are ready for consumption. 
We run all our experiments on a single machine running Ubuntu $16.04$ with $60$GB RAM and $12$ cores. 
For all performance related experiments, we measure $5$ runs and report the mean of the three observations that are closest to the median. 
To normalize the numeric features, we set $H = 1000$. Unless mentioned explicitly, we set $\gamma \rightarrow 0$.

\subsection{Experiments on AdHoc Workload} \label{sec:exp}

In this section, we study the impact of different algorithms on the metrics, explore the effect of parameter $\gamma$ on the objective function, study the impact of algorithmic optimization and provide empirical evidence of scalability to large datasets.

\subsubsection{Effect of Algorithm Used} \label{sec:algo}


\begin{figure*}[t]
    \begin{subfigure}{0.3\linewidth}
    \includegraphics[scale=0.65]{figures/fixedsummaryvaryingworkloadtime.pdf}
    \caption{Runtime with varying workload size, |S|=100} \label{fig:opt1}
    \end{subfigure}
    \hspace{0.5em}
    \begin{subfigure}{0.3\linewidth}
    \includegraphics[scale=0.65]{figures/fixedworkloadvaryingsummary.pdf} 
    \caption{Runtime with varying summary size, |W|=5000} \label{fig:opt2}
    \end{subfigure}
    \hspace{0.5em}
    \begin{subfigure}{0.3\linewidth}
    \includegraphics[scale=0.65]{figures/fixedsummaryvaryingworkloadprunedratio.pdf} 
    \caption{Pruning ratio with varying workload size, |S|=100} \label{fig:opt3}
    \end{subfigure}
    
    \begin{subfigure}{0.3\linewidth}
    \includegraphics[scale=0.65]{figures/fixedworkloadvaryingsummaryprunedratio.pdf} 
    \caption{Pruning ratio with varying\\summary size, |W|=5000} \label{fig:opt4}
    \end{subfigure}
    \begin{subfigure}{0.3\linewidth}
    \includegraphics[scale=0.65]{figures/runtime.pdf}
    \caption{Scalability with varying workload size, |S|=$\sqrt{|W|}$} \label{fig:scalability:exp1}
    \end{subfigure}
    \hspace{0.5cm}
    \begin{subfigure}{0.3\linewidth}
    \includegraphics[scale=0.65]{figures/runtimefixedworkload.pdf}
    \caption{Scalability with varying summary size, |W|=5000} \label{fig:scalability:exp2}
    \end{subfigure}
    \caption{Impact of performance optimizations and scalability experiments}
\end{figure*}

We first evaluate the runtime behavior of different algorithms. 
In order to benchmark runtime performance, we perform summarization over $5000$ randomly chosen \texttt{AdHoc} queries whose feature vectors have already been materialized. The summary size of the workload varies from $50$ to $1000$.
Figure~\ref{fig:timetaken} shows the runtime of the implemented algorithms. 
For k-medoids and the applied hierarchical algorithm (average linkage), we use the euclidean distance over numeric features as the distance metric. 
Further, we report the runtimes of the algorithms when we exclusively use either categorical or numeric features. 

The first observation is that using clustering algorithms with categorical features is the most expensive choice (time $> 10,000$ seconds). 
The reason is that even though feature vectors have been materialized, finding the Jaccard distance is $O(\norm{\bq})$ time as compared to $O(1)$ for the distance computation when single valued numeric feature metrics are used. 
Further, in order to find the medoid of each cluster, the number of operations required is quadratic in the cluster size which amplifies the performance difference. 
We also employed optimizations such as caching the distance between every pair of queries once it is computed and pre-computing the distance matrix (which is already $O(n^2)$). 
For both modifications, we observed an improvement in runtime by an order of magnitude but the asymptotic quadratic behaviour does not change. 
Specifically, increasing the size of the input workload to $15000$ is sufficient to offset the gains introduced by the optimizations. 

Our second observation focuses on the decreasing runtime for clustering if the k-medoids algorithm is applied. 
When the summary size is small, i.e.,~the number of desired clusters is small, most of the queries may be concentrated in a few clusters. 
Then, the overall runtime of the algorithm is dominated by finding the medoid for such clusters. As the summary size increases, cluster skew reduces which improves the runtime. 
This effect is further amplified when the chosen summary size is of the same order as the input workload as most of the queries are chosen as initial cluster centers. 
In contrast, if the summary size is equivalent to the input workload size, clustering will happen in a single pass of the input. 
Compared to clustering algorithms whose performance depends heavily on whether categorical or numeric or both features are used, the submodular algorithm is less sensitive to the chosen features since the submodular gain computation depends on a single query.
%We observe that the submodular algorithm does not exhibit a large performance variance when using categorical or numeric features exclusively since each submodular gain computation depends only on a single query. 

\subsubsection{Representativity and Coverage}
Next, we compare the metrics for the same set of $5000$ queries used in section~\ref{sec:algo} and fix $\td(\cdot)$ to be the input distribution. 
Figure~\ref{fig:repcov} shows the metrics for all algorithms. 
In line with expectation, random sampling has the best representativity score and the lowest coverage. 
All clustering algorithms perform poorly on the representativity metric but achieve good coverage. 
This is not surprising considering the fact that the cluster initialization step identifies {\em outlier} queries as cluster centers, since they have the largest distance from most other queries. In turn, this ensures high coverage as queries close to outliers are present in the summary. 
Our submodular algorithm has a slightly lower coverage compared to the best clustering algorithms, but performs well on representativity. 
Note that since $\gamma \rightarrow 0$, the submodular algorithm focuses on maximizing coverage first, and for the chosen input workload of $100$ queries is not able to cover the active domain. 
Once the best possible coverage is achieved for the fixed $\gamma$, $\rho$ should improve even further.



\subsubsection{Trade-off between Metrics}

\begin{figure}[!htp]
    \includegraphics[scale=1]{figures/tradeoff.pdf}
    \caption{Trade-off between metrics for varying summary sizes}
    \label{fig:smooth}
\end{figure}

In the next experiment, we empirically verify the impact of the $\gamma$ parameter and study how it can be used to trade-off between the two metrics. 
Figure~\ref{fig:smooth} shows the trade-off as the value of $\gamma$ decreases from $1$ to $0$. 
Observe that as $\gamma$ decreases, representativity starts dropping and coverage starts to increase. 
Note that the increase in coverage or decrease in representativity need not be monotone. This may happen because of the complex interaction between features. 
Since all features are uniformly weighted, features with more tokens tend to dominate both $\alpha$ and $\rho$. 
In order to balance that, we can set the weight for each feature inversely proportional to its active domain. 
However, in almost all our experiments, no feature dominated a different feature even when each feature had the same weight. In other words, the representativity score for each feature shows an empirical monotone behavior as $\gamma$ changes.
Table~\ref{tradeoff:prod} shows the impact of $\gamma$ on summarization for a day's workload of a specific user on System X.
The input contains $512796$ queries and the generated summary consists of $1000$ queries. As the value of $\gamma$ decreases, $\rho_{1}$ increases at the expense of $\alpha_{\mathit{avg}}$. Using the generated summary, we are able to identify recurring patterns in the input workload.


 \begin{table}
	\scriptsize
	
	\scalebox{0.95}{
	\begin{tabular}{ c|l|l|l|l|l|l|l}
		\toprule[0.1em]
		$\gamma$ & $f^s_1$ &  $f^p_1$ &  $f^p_2$ & $f^p_4$ & $f^p_5$  \\ \midrule[0.1em]
		$10^0$ & $ 0.75 \mid 1.0 $ & $ 0.67\mid 1.0$ & $ 0.57\mid 1.0$ & $0.9\mid 1.0$ & $0.5\mid 1.0$  \\ \midrule
		$10^{-3}$ & $ 0.76\mid 1.0$ & $0.74\mid 0.81$ & $ 0.66\mid 0.88$  & $0.90\mid 1.0$ & $0.6\mid 0.84$  \\		\midrule
		$10^{-10}$ & $ 0.8\mid 1.0$ & $ 0.81\mid 0.68$ & $ 0.73\mid 0.75$ & $ 0.90\mid 1.0$ & $0.69\mid 0.70$  \\	\midrule
		$10^{-15}$ & $ 0.84\mid 1.0$ & $0.87\mid 0.57$ & $0.80\mid 0.61$ & $ 0.95\mid 0.56$ & $ 0.74\mid 0.64$  \\	\midrule
		$10^{-20}$ & $ 0.88\mid 1.0$ & $0.98\mid 0.32$ & $0.94\mid 0.26$ & $ 0.98\mid 0.30$ & $ 0.94\mid 0.18$  \\	\midrule
		$10^{-25}$ & $ 0.91\mid 1.0$ & $0.99\mid 0.07$ & $0.94\mid 0.07$ & $ 0.98\mid 0.07$ & $ 0.99\mid 0.02$  \\
		\bottomrule
	\end{tabular}}
	\caption{Tradeoff between metrics for production workload. Each cell shows $\rho_{1} \mid \alpha_{\mathit{avg}}$} \label{tradeoff:prod}
\end{table}

\begin{figure*}[!htp]
\hspace{-1cm}
    \begin{subfigure}{0.45\linewidth}
    \includegraphics[scale=1]{figures/tpchuniformkmedoids.pdf}
    \caption{k-medoids on uniform TPC-H workload} \label{fig:tpch:exp1}
    \end{subfigure}
    \hspace{1cm}
    \begin{subfigure}{0.45\linewidth}
    \includegraphics[scale=1]{figures/tpchuniformsubmodular.pdf}
    \caption{Submodular algorithm on uniform TPC-H workload} \label{fig:tpch:exp2}
    \end{subfigure}
    \caption{Performance metrics for uniform TPC-H workload}
\end{figure*}


\subsubsection{Algorithmic Optimizations} 
This experiment tests the efficiency of the {\em early exit} optimization technique applied for our submodular algorithm and its effect on runtime. 
As previously, we use a $5000$-query subset of the \texttt{AdHoc} dataset. 
We omit reporting the time spent by our basic greedy algorithm because it is much slower than after applying our proposed optimization techniques. 
Figure~\ref{fig:opt1} and Figure~\ref{fig:opt2} show how the two optimization techniques scale with respect to the input workload size (when summary size is kept fixed to $100$) and the summary workload size (when input workload is fixed to $5000$ queries). 
The effect of early exit optimization increases as the dataset size increases. 
This is because early exit prunes away a lot of computation in each iteration of the greedy process. 
To further investigate early pruning, let $\texttt{iter}_{\textit{total}}$ be the total number of iterations in the greedy process without any optimizations and $\texttt{iter}_{\textit{exit}}$ be the number of iterations performed by the algorithm with the early exit optimization switched on. 
Then, the pruning ratio $\texttt{iter}_{\textit{exit}}/\texttt{iter}_{\textit{total}}$ quantifies the effectiveness of the strategy. 
Figure~\ref{fig:opt3} and Figure~\ref{fig:opt4} show the impact of varying workload and summary sizes on the pruning ratio. 
As the workload size increases, the effectiveness of the optimization also increases indicating that the submodular bound becomes tighter and thus more effective. 
With respect to the summary workload size, the fraction of iterations pruned remains uniform and eventually decreases for large summaries.

\subsubsection{Scalability} In order to benchmark scalability, we execute the algorithm on a single thread on a single machine and use all categorical and numeric features for metrics computation. 
Figure~\ref{fig:scalability:exp1} shows the runtime in minutes when the input workload size $n$ varies and the summary size is fixed to $\sqrt{n}$. 
The largest workload of size $2.4$ million takes $60$ minutes to run and we generally observe a linear increase in runtime when increasing the workload size. 
Figure~\ref{fig:scalability:exp2} shows varying summary size while keeping the input workload fixed at $2$ million. 
Here, generating a summary with $12000$ queries takes roughly $6$ hours and we observe a linear increase in runtime with an increase in summary size again.


\subsection{Experiments on TPC-H Workload}
In this part of the evaluation, we compare our algorithm with k-medoids by carefully constructing workloads where clustering performs the best and then understand the strengths and limitations of our proposed approach. 


\begin{figure*}[!htp]
    \begin{subfigure}{0.3\linewidth}
    \includegraphics[scale=0.7]{figures/tpchkmedoidstwometrics.pdf}
    \caption{k-medoids} \label{fig:tpch2:exp1}
    \end{subfigure}
	\hspace{1em}
    \begin{subfigure}{0.3\linewidth}
    \includegraphics[scale=0.7]{figures/tpchsubmodulartwometrics.pdf}
    \caption{Submodular} \label{fig:tpch2:exp2}
    \end{subfigure}
	\hspace{1em}
    \begin{subfigure}{0.3\linewidth}
    \includegraphics[scale=0.7]{figures/zipftpchdeskewfunccall.pdf}
    \caption{Skewed TPC-H workload} \label{fig:tpch2:exp3}
    \end{subfigure}
    \caption{Evaluation of the TPC-H benchmark using categorical features only.}
\end{figure*}

\smallskip
\noindent \introparagraph{Uniform Workload} For our first experiment, we construct a workload with $418$ queries where each TPC-H template is instantiated $19$ times. 
Each instantiation generates different constants in the query which affects the execution statistics. 
Then, we ask both the algorithms to generate summaries ranging from $1$ to $44$ in size. 
Our goal is observe how the different metrics change as the workload size increases. 
To create the summaries, all categorical and numeric metrics introduced in Section~\ref{subsec:encoding} are computed. \anja{Figure~\ref{fig:tpch:exp1}}{Is this missing some values?} Figure~\ref{fig:tpch:exp2} shows all metrics for this experiment. 
In both cases, the coverage metric shows monotonic behavior. 
The submodular algorithm has a strictly better coverage than k-medoids at each step since it is trying to maximize coverage (recall that $\gamma \rightarrow 0$). 
However, k-medoids has a better performance for the $\rho$ metric. 
It reaches a maximum when query size is $22$ and then marginally decreases until query $33$ before increasing again. 
This behavior is expected since the initialization step of k-medoids chooses cluster center for $C_i$ by finding a query that has the largest distance from cluster center of $C_{i-1}$. 
For the TPC-H workload, all queries are {\em outliers} with respect to each other and therefore, centers are chosen perfectly. 
On the other hand, the submodular algorithm tries to maximize coverage by including at least one instance of each template until $20$ and $\rho_1$ reaches a maximum at that size. 
It does not pick an instance of $Q_{14}$ and $Q_{6}$ because their tokens have already been covered by other queries. 
One may find it surprising that there is not much variation in the $\rho$ metrics after $22$ and the low overall coverage. 
The main reason for this is the wide variability in runtime statistics for different instantiations of the same query template. 
To confirm this hypothesis, we calculate $\alpha$ and $\rho$ over categorical features only as shown in Figure~\ref{fig:tpch2:exp1} and Figure~\ref{fig:tpch2:exp2}. 
Here, the categorical feature coverage for both algorithms reaches $1$ in at most $22$ queries. 
Figure~\ref{fig:tpch2:exp1} demonstrates the observation from example~\ref{ex:non-monotone} much more clearly. 
Here the $\rho_1$ score achieves a local maxima when the summary size is a multiple of $22$. 
The submodular algorithm behaves differently: After maximizing coverage, it picks queries according to the objective function and ensuring that queries are chosen such that the $q(\cdot)$ distribution is maintained. 
Specifically, for workload sizes between $20$ and $77$, the algorithm will always return $20$ queries as that summary size has the highest score \footnote{The greedy algorithm never picks $Q_1$ and $Q_6$ because most of its feature values are covered by other queries.}.
Beyond $77$,the $\rho_1$ score of summary size $20$ is exceeded and increases in each iteration, thus, those will be returned. 
Both algorithms eventually reach $\rho_1 = 1$ with an increase in summary size. 

So far, we have used uniform weights for all features. 
We observed in some of our experiments that the metrics can be significantly improved by assigning a higher weight to a feature that has lower $\rho$ or $\alpha$. 
We use this heuristic to perform a few weight transfer iterations by lowering the weight of features with high metrics and transferring it to features with low metrics. 
Using this technique, we were able to boost the metrics to $\rho_1 = 0.84, \rho_\infty = 0.44, \alpha_{\mathit{avg}} = 0.82, \alpha_{\mathit{min}} = 0.31$ when summary size is $22$ which is strictly better than k-medoids scores of $\rho_1 = 0.75, \rho_\infty = 0.34, \alpha_{\mathit{avg}} = 0.70, \alpha_{\mathit{min}} = 0.22$.

\smallskip
\noindent \introparagraph{Skewed Workload} Our next experiment verifies the behavior of fixing $\td(\cdot)$ to a user specified distribution. 
For this experiment, we generate a skewed TPC-H workload where query template $Q_i$ is instantiated $\lfloor \frac{1}{i+1} \cdot 66 \rfloor$ times. 
Since $Q_1$ contains \texttt{ \color{blue}SUM, MAX, COUNT}, it dominates the function calls in the workload whereas \texttt{ \color{blue}SUBSTR} and \texttt{ \color{blue} ARRAY-AGG} are present only in $Q_{22}$ and $Q_{19}$ respectively. 
To keep the setting simple, we set $\td(\cdot)$ for function call feature to be uniform, i.e,~$0.2$ for each function call token (as the domain of function call feature has $5$ values) and calculate $\rho_1, \alpha_{\mathit{avg}}$ only for function call feature. 
Figure~\ref{fig:tpch2:exp3} shows the metrics as a function of the summary workload size. 
The first query picked by our algorithm is $Q_1$ since it has the most function call tokens. 
The next two queries are $Q_{19}$ and $Q_{22}$ to cover the remaining two tokens. 
After another round of the same sequence, all remaining queries picked are $Q_1$ and as the summary size grows, \texttt{ \color{blue}SUM, MAX, COUNT} dominate the summary workload. 
Thus, the algorithm will return a summary size of $3$ with one instance each of $Q_1, Q_{19}, Q_{22}$ that covers all tokens and has the maximum $\rho_1$.  

\subsection{Discussion} So far, we have observed how different knobs and configuration parameters impact various performance metrics. 
The goal of this work is to develop a general enough framework that can capture most of the cases where a succinct workload is of great use. 
However, much remains to be explored before we utilize the full power of the framework. 
Key among these questions is how to choose which features are required to generate a good summary. 
The answer is partly dependent on the chosen application and partly on how the features interact with each other. 
While adding more features to the problem certainly provides more information, it is not necessary that adding more features will give a better result. 
For instance, the addition of more features will require a larger summary size to increase the coverage which in turn can possibly decrease representativity. 
A more principled approach on feature engineering is certainly beneficial. 
This also points us to the use of {\em higher order features} in our framework. 
For instance, one could create a second degree feature that captures the occurrence of $\langle t_1, t_2 \rangle$ where $t_1$ and $t_2$ are tokens of two different features. 
This can potentially help us generate even better summaries since it captures more fine-grained cross feature information. 
We conclude the section with the following heuristics that work well in practice from our experience:

\begin{packed_enum}
    \item If representativity is more important than coverage, take a sample first and then remove queries using the greedy algorithm to improve coverage.
    \item The use case dictates which (combination of) features should be used for summarization.
    %Choose the better summary where either categorical features are used or numeric features are used as baselines.
    \item Perform weight transfer iterations to further boost the scores.
    \item If the domain of features is large, set $\gamma$ closer to $1$ to dampen the effect of coverage.
\end{packed_enum}
